Reinforcement Learning Informed Evolutionary Search for Autonomous Systems Testing

Evolutionary search-based techniques are commonly used for testing autonomous robotic systems. However, these approaches often rely on computationally expensive simulator-based models for test scenario evaluation. To improve the computational efficiency of the search-based testing, we propose augmenting the evolutionary search (ES) with a reinforcement learning (RL) agent trained using surrogate rewards derived from domain knowledge. In our approach, known as RIGAA (Reinforcement learning Informed Genetic Algorithm for Autonomous systems testing), we first train an RL agent to learn useful constraints of the problem and then use it to produce a certain part of the initial population of the search algorithm. By incorporating an RL agent into the search process, we aim to guide the algorithm towards promising regions of the search space from the start, enabling more efficient exploration of the solution space. We evaluate RIGAA on two case studies: maze generation for an autonomous ant robot and road topology generation for an autonomous vehicle lane keeping assist system. In both case studies, RIGAA converges faster to fitter solutions and produces a better test suite (in terms of average test scenario fitness and diversity). RIGAA also outperforms the state-of-the-art tools for vehicle lane keeping assist system testing, such as AmbieGen and Frenetic.

==> algorithms/diversity.tex <==
\begin{algorithm}
\caption{Calculate Average Diversity}\label{avgdiv}
\begin{algorithmic}[1]
\Procedure{Calculate Average Diversity}{$S = {s_1, s_2, ..., s_N}$}
\State $sum \gets 0$
\For{$i \gets 1$ to $N$}
\For{$j \gets i+1$ to $N$}
\State $sum \gets sum + diversity(s_i, s_j)$
\EndFor
\EndFor
\State $avgDiversity \gets \frac{sum}{\binom{n}{2}}$ \Comment{Calculate average}
\State \textbf{return} $avg$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> algorithms/diversity2.tex <==
\begin{algorithm}[H]
\caption{Calculate Average Diversity}
\begin{algorithmic}[1]
\Procedure{AverageDiversity}{$elements$}
    \State $diversity \gets 0$
    \State $n \gets \text{length}(elements)$ \Comment{Calculate number of elements}
    \For{$i \gets 1$ \textbf{to} $n$}
        \For{$j \gets i+1$ \textbf{to} $n$}
            \If{$elements_i \ne elements_j$}
                \State $diversity \gets diversity + 1$
            \EndIf
        \EndFor
    \EndFor
    \State $avgDiversity \gets \frac{diversity}{\binom{n}{2}}$ \Comment{Calculate average}
    \State \textbf{return} $avgDiversity$
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> algorithms/f2.tex <==
\begin{algorithm}
\caption{Calculate individual novelty}\label{alg:f2}
\begin{algorithmic}[1]
\Procedure{CalculateNovelty}{$ {ts_{in}, ts_1, ts_2, ..., ts_N}, N$}
\State $sum \gets 0$
\For{$i \gets 1$ to $N$}
\State $sum \gets sum + diversity(ts_{in}, ts_i)$
\EndFor
\State $F_2 \gets \frac{sum}{N}$ \Comment{Calculate average}
\State \textbf{return} $F_2$
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> tables/rq2_veh_mean.tex <==
\begin{table}[H]
\caption{Mean values of test suite fitness and diversity for different values of $\varepsilon$}
\label{tab:sweep_values}
\centering
    \begin{tabular}{ccccccc}
    \hline
        Problem & Metric & 0.2 & 0.4 & 0.6 & 0.8 & 1 \\ \hline
        robot & Mean fitness & 205.712 & 207.856 & 208.304 & 211.414 & 213.68 \\ 
        robot & Mean diversity & 0.775 & 0.782 & 0.773 & 0.78 & 0.771 \\ 
        vehicle & Mean fitness & 8.976 & 9.075 & 9.045 & 8.842 & 9.119 \\ 
        vehicle & Mean diversity & 0.812 & 0.813 & 0.809 & 0.816 & 0.801 \\ \hline
    \end{tabular}
\end{table}

==> tables/rq3_effect_size_rob.tex <==
\begin{table}[H]
\caption{Non parametric test results and effect sizes for the test suites generated by different approaches for autonomous robot problem}
\label{tab:algo_rob_effect}
\centering
\scalebox{0.9}{
    \begin{tabular}{llllllllll}
    \hline
        Metric & A & B & p-value & Effect size & Metric & A & B & p-value & Effect size \\ \hline
        fitness & Random & NSGA-II & 0.000 & -1.0, L & diversity & Random & NSGA-II & 0.000 & 1.0, L \\ 
        ~ & Random & RIGAA & 0.000 & -1.0, L & ~ & Random & RIGAA & 0.000 & 1.0, L \\ 
        ~ & NSGA-II & RIGAA & 0.000 & -0.483, L & ~ & NSGA-II & RIGAA & 0.000 & -0.632, L \\ \hline
    \end{tabular}}
\end{table}

==> tables/rq3_effect_size_veh.tex <==
\begin{table}[H]
\caption{Non parametric test results and effect sizes for the test suites generated by different approaches for autonomous vehicle problem}
\label{tab:algo_veh_effect}
\centering
\scalebox{0.9}{
    \begin{tabular}{llllllllll}
    \hline
        Metric & A & B & p-value & Effect size & Metric & A & B & p-value & Effect size \\ \hline
        fitness & Random & NSGA-II & 0.000 & -0.978, L & diversity & Random & NSGA-II & 0.000 & 1.0, L \\ 
        ~ & Random & RIGAA & 0.000 & -0.994, L & ~ & Random & RIGAA & 0.000 & 1.0, L \\ 
        ~ & NSGA-II & RIGAA & 0.000 & -0.726, L & ~ & NSGA-II & RIGAA & 0.264 & -0.196, S \\ \hline
    \end{tabular}}
\end{table}

==> tables/rq3_means.tex <==

\begin{table}[H]
\caption{Non parametric test results and effect sizes for the test suites generated by different approaches for autonomous vehicle problem}
\label{tab:algo_veh_rob_mean}
\centering
    \begin{tabular}{lllll}
    \hline
        Problem & Metric & Random & NSGA-II & RIGAA \\ \hline
        robot & mean fitness & 81.29177163 & 182.4904647 & 197.0335834 \\ 
        robot & mean diversity & 0.933862876 & 0.683762476 & 0.728063143 \\ 
        vehicle & mean fitness & 3.442476974 & 6.252650098 & 9.488573475 \\ 
        vehicle & mean diversity & 0.96224624 & 0.726609126 & 0.747239542 \\ \hline
    \end{tabular}
\end{table}

==> tables/rq4.tex <==
 \begin{table}[H]
\caption{Comparing random and RL based generators in terms of quality and diversity of the solutions for the vehicle model in simulation}
\label{tab:full_gen}
\centering
    \begin{tabular}{lllll}
    \hline
        Metric & Random & RL agent & p-value & Effect size \\ \hline
        mean fitness & 0.246 & 0.7 & 0.000 &0.819,L\\ %\hline
        mean diversity & 0.955 & 0.701 & 0.000 & 1.0,L \\ \hline
    \end{tabular}
\end{table}

==> tables/rq5_effect.tex <==
 \begin{table}[H]
\caption{Comparing random and RL based generators in terms of quality and diversity of the solutions for the vehicle model in simulation}
\label{tab:full_gen}
\centering
\scalebox{0.9}{
    \begin{tabular}{llllllllll}
    \hline
        Metric & A & B & p-value & Effect size & Metric & A & B & p-value & Effect size \\ \hline
        fitness & Random & NSGA-II & 0.000 & -0.818, L & diversity & Random & NSGA-II & 0.000 & 1.0, L \\ 
        ~ & Random & RIGAA & 0.000 & -0.901, L & ~ & Random & RIGAA & 0.000 & 1.0, L \\ 
        ~ & NSGA-II & RIGAA & 0.000 & -0.438, M & ~ & NSGA-II & RIGAA & 0.149 & 0.382, M \\ \hline
    \end{tabular}}
\end{table}

==> tables/rq5_mean.tex <==

\begin{table}[H]
\caption{Mean fitness and diversity of the test suites produced for the autonomous vehicle model in the simulator}
\label{tab:algo_veh_rob_mean}
\centering
    \begin{tabular}{llll}
    \hline
        Metric & Random & NSGA-II & RIGAA \\ \hline
        mean fitness & 0.31 & 0.807 & 0.906 \\ 
        mean diversity & 0.953 & 0.806 & 0.749 \\ \hline
    \end{tabular}
\end{table}
